ORA3D: Overlap Region Aware Multi-view 3D Object Detection

Current multi-view 3D object detection methods often fail to detect objects in the overlap region properly, and the networks' understanding of the scene is often limited to that of a monocular detection network. Moreover, objects in the overlap region are often largely occluded or suffer from deformation due to camera distortion, causing a domain shift. To mitigate this issue, we propose using the following two main modules: (1) Stereo Disparity Estimation for Weak Depth Supervision and (2) Adversarial Overlap Region Discriminator. The former utilizes the traditional stereo disparity estimation method to obtain reliable disparity information from the overlap region. Given the disparity estimates as supervision, we propose regularizing the network to fully utilize the geometric potential of binocular images and improve the overall detection accuracy accordingly. Further, the latter module minimizes the representational gap between non-overlap and overlapping regions. We demonstrate the effectiveness of the proposed method with the nuScenes large-scale multi-view 3D object detection data. Our experiments show that our proposed method outperforms current state-of-the-art models, i.e., DETR3D and BEVDet.

==> tex/discussion.tex <==
Here, we discuss several exciting future research avenues that can address current limitations of our method. While the disparity estimation network outputs dense disparity maps for each view, we do not explicitly utilize the estimated disparities for 3D object detection. We rather use the disparity estimation network as an intermediate medium that allows the image backbone network to extract 3D aware image features for overlapping regions as shown in Fig.~\ref{fig:figure2}. Although we have shown that such indirect guidance already adds performance improvement to the object detection head, explicit utilization of the estimated disparity maps or depth maps would give us better performance. As a future work, we would like to improve the performance of the stereo matching network and integrate the network with the object detection head for better utilization of the estimated disparities. 
% As mentioned, instead of a dense depth map, we use a stereo disparity map obtained from the overlap region to utilize 3D information of the multi-view scenes for 3D detection network. This significantly improves the accuracy of the 3D detection pipeline. Therefore, there is plenty of room for performance improvement if the dataset contains the dense depth map to inform dense 3D geometric and uses the dense depth map to replace stereo disparity map estimation with dense map estimation on the overlap region. 
% In terms of training computation complexity, many 3D object detection methods rely on CBGS~\cite{zhu2019class} to improve the performance, regardless of increasing computation complexity approximately four times. However, our proposed method achieves state-of-the-art results without using CBGS method.
